Popularity on the 3D-Euclidean Stable Roommates

We study the 3D-Euclidean Multidimensional Stable Roommates problem, which asks whether a given set $V$ of $s\cdot n$ agents with a location in 3-dimensional Euclidean space can be partitioned into $n$ disjoint subsets $\pi = \{R_1 ,\dots , R_n\}$ with $|R_i| = s$ for each $R_i \in \pi$ such that $\pi$ is (strictly) popular, where $s$ is the room size. A partitioning is popular if there does not exist another partitioning in which more agents are better off than worse off. Computing a popular partition in a stable roommates game is NP-hard, even if the preferences are strict. The preference of an agent solely depends on the distance to its roommates. An agent prefers to be in a room where the sum of the distances to its roommates is small. We show that determining the existence of a strictly popular outcome in a 3D-Euclidean Multidimensional Stable Roommates game with room size $3$ is co-NP-hard.

==> sections/generalization.tex <==
\section{Generalizing room size}


==> sections/mixedpopularity.tex <==
\section{Mixed Popularity}\label{mixedpop}

==> sections/mixedpopularityv2.tex <==
\section{Mixed Popularity}\label{mixedpop}
We show that a mixed popular outcome is guaranteed to exist in any roommate diversity game. However, a mixed popular outcome for a roommate diversity game cannot be computed in polynomial time, even if the preferences are dichotomous, unless P=NP.

%To show the guaranteed existence, we use the minimax theorem \cite{v.Neumann1928}. To demonstrate hardness, we construct a reduction from the X3C problem to the roommate diversity problem. This reduction is similar to the reduction in \cref{strictpop}.

\begin{theorem}
	Any roommate diversity game is guaranteed to have a mixed popular outcome.
\end{theorem}
\begin{proof}
Every roommate diversity game can be viewed as a finite two-player symmetric zero-sum game where the rows and columns of the game matrix are indexed by all possible outcomes $\pi_1, \dots, \pi_{t}$ and the entry at $(i,j)$ of the game matrix has value $\phi(\pi_i,\pi_j)$. By the minimax theorem \cite{v.Neumann1928}, we have that the value of this game is 0. Therefore, any maximin strategy is popular.
\qed\end{proof}

To show that a mixed popular outcome for a roommate diversity game cannot be computed in polynomial time, we change the reduction of strict popularity in \cref{strictpop} by doubling the agents, adding new agents, and changing the room size and preference profiles accordingly. These additions ensure that the monolithic outcome is strictly popular if $(X,C)$ has no solution and that the monolithic outcome is not popular if $(X,C)$ has a solution. The full reduction can be found in the appendix or the full paper.

==> sections/popularity.tex <==
\section{Popularity}
\subsection{No guaranteed existence}

==> sections/popularityv2.tex <==
\section{Popularity}
In this section we show that a popular outcome is not guaranteed to exist in a roommate diversity game. %To demonstrate this, we provide a roommate diversity game in which no popular outcome exists.

Let $R = \left\{r_1,r_2,r_3\right\}$ and $B = \left\{b_1,b_2,b_3,b_4,b_5,b_6\right\}$. Consider the roommate diversity game $\overline{G} = (R,B,3,(\succsim_a)_{a\in R\cup B})$ with the following trichotomous preference profiles: %with the their trichotomous preference profiles described in \cref{nopopgame}.

%\begin{table}[h!]
\begin{center}
	\begin{tabular}{ | l | l | l | l | }
		\hline
		\multirow{2}{*}{Agent} & \multicolumn{3}{c|}{Preference Profile}  \\\cline{2-4}
		& $D_a^+$ & $D_a^n$ & $D_a^-$  \\\hline
		$a = r_1$ & $\left\{\frac{1}{3}\right\}$ & & $\left\{\frac{2}{3}, \frac{3}{3}\right\}$  \\  
		$a \in \left\{r_2,r_3\right\}$ & $\left\{\frac{2}{3}\right\}$ & & $\left\{\frac{1}{3}, \frac{3}{3}\right\}$  \\\hline\hline
		
		$a \in \left\{b_1,b_2,b_3,b_4\right\}$ & $\left\{\frac{1}{3}\right\}$ & $\left\{\frac{2}{3}\right\}$ & $\left\{\frac{0}{3}\right\}$ \\
		$a \in \left\{b_5,b_6\right\}$ & $\left\{\frac{0}{3}\right\}$ & & $\left\{\frac{1}{3}, \frac{2}{3}\right\}$\\\hline
	\end{tabular}
	%\caption{Preference profile $(\succsim_a)_{a \in R \cup B}$.}\label{nopopgame}
\end{center}
%\end{table}
Let us define the rooms $P_1 = \left\{r_1, \hat{b}_1, \hat{b}_2\right\}; P_2 = \left\{r_2,r_3,\hat{b}_3\right\}; P_3 = \left\{b_5,b_6,\hat{b}_4\right\},$
where $\hat{b}_1,\hat{b}_2,\hat{b}_3,\hat{b}_4 \in \left\{b_1,b_2,b_3,b_4\right\}$. An outcome $\pi_{top}$ is called a top-type outcome if we can write $\pi_{top} = \left\{P_1, P_2, P_3\right\}$. We can show that for any non-top-type outcome $\pi$, a top-type outcome $\pi'$ exists such that $\pi'$ is strictly more popular than $\pi$. However, for any top-type outcome $\pi'$, we can construct another top-type outcome $\pi''$ such that $\pi''$ is strictly more popular than $\pi'$. Thus, no outcome in this roommate diversity game is popular.
%See appendix or full paper for the lemmas and theorem which show that $\overline{G}$ has no popular outcome. 
\begin{lemma}\label{popnotgar2more}
	For any outcome $\pi$ of $\overline{G}$, we have that there are at least 2 agents in a room with a fraction that it does not approve of. %That is, for any outcome $\pi$ of $\overline{G}$, 
	%$|D_\pi^n \cup D_\pi^-| \geq 2.$
\end{lemma}
\begin{proof}
	To derive a contradiction, assume that there exists an outcome $\pi$ of $\overline{G}$ such that $|D_\pi^n \cup D_\pi^-| < 2$. Consider the following cases.
	\begin{enumerate}
		\item $|D_\pi^n \cup D_\pi^-| = 0$.\\
		Then $b_1,b_2,b_3,b_4 \in D_\pi^+$, therefore each of $b_1,b_2,b_3,b_4$ must be in a room with fraction $\frac{1}{3}$. We require at least 2 rooms $S_1,S_2$ with fraction $\frac{1}{3}$ so that each of $b_1,b_2,b_3,b_4$ is contained in a room with fraction  $\frac{1}{3}$. There is exactly 1 red agent that approves of fraction $\frac{1}{3}$, namely $r_1$. Thus, $S_1$ or $S_2$ must contain a red agent $r$ that does not approve of fraction $\frac{1}{3}$. Thus, $|D_\pi^n \cup D_\pi^-| \geq 1$ in this case as $r \in D_\pi^-$. This contradicts $|D_\pi^n \cup D_\pi^-| = 0$.
		
		\item $|D_\pi^n \cup D_\pi^-| = 1$.\\
		Let us write $D_\pi^n \cup D_\pi^- = \left\{a\right\}$. Consider the following cases regarding $a$.
		\begin{enumerate}[\theenumi.1.]
			\item $a = r_1$.\\
			Then $b_1,b_2,b_3,b_4 \in D_\pi^+$, therefore each of $b_1,b_2,b_3,b_4$ must be in a room with fraction $\frac{1}{3}$. We require at least 2 rooms $S_1,S_2$ with fraction $\frac{1}{3}$ so that each of $b_1,b_2,b_3,b_4$ is contained in a room with fraction  $\frac{1}{3}$. There is exactly 1 red agent that approves of fraction $\frac{1}{3}$, namely $r_1$. Thus, $S_1$ and $S_2$ both must contain a red agent $r, r' \in R$ that do not approve of fraction $\frac{1}{3}$. Thus, $|D_\pi^n \cup D_\pi^-| \geq 2$ as $r,r' \in D_\pi^-$. This contradicts $|D_\pi^n \cup D_\pi^-| = 1$.
			
			\item $a \in \left\{r_2,r_3\right\}$.\\
			W.l.o.g. assume that $a = r_2$. We have that $r_3 \in D_\pi^+$, thus the room $S$ that contains $r_3$ must be of fraction $\frac{2}{3}$. There are exactly 2 agents that approve of fraction $\frac{2}{3}$, namely $r_2$ and $r_3$. Since $r_2 \notin S$, as $r_2 \in D_\pi^-$, the room $S$ must contain a red agent $r \neq r_2$ such that $r \in D_\pi^-$. Thus, $|D_\pi^n \cup D_\pi^-| \geq 2$ in this case as $r_2,r \in D_\pi^-$. This contradicts $|D_\pi^n \cup D_\pi^-| = 1$.
			
			
			\item $a \in \left\{b_1,b_2,b_3,b_4\right\}$.\\
			Analogous to case 2.1.
			
			\item $a \in \left\{b_5,b_6\right\}$.\\
			Analogous to case 2.1.\qed
			
		\end{enumerate}
	\end{enumerate}
	\end{proof}

\begin{lemma}\label{popnotgartopcard}
	For any outcome $\pi$ of $\overline{G}$, if $|D_\pi^n| = 1$ and $|D_\pi^-| = 1$, then $\pi$ is a top-type outcome. %That is, for any outcome $\pi$ of $\overline{G}$, 
	%$$|D_\pi^n| = 1 \wedge |D_\pi^-| = 1 \implies \pi \text{ is a top-type outcome.}$$
\end{lemma}
\begin{proof}
	Let $\pi$ be an outcome such that $|D_\pi^n| = 1$ and $|D_\pi^-| = 1$. Let us write $D_\pi^n = \left\{a^n\right\}$ and $|D_\pi^-| = \left\{a^-\right\}$. Since the agents in $\left\{b_1,b_2,b_3,b_4\right\}$ are the only agents with a non-empty corresponding $D_a^n$, we have that $a^n \in \left\{b_1,b_2,b_3,b_4\right\}$. 
	
	To derive a contradiction, assume that $a^- \notin \left\{b_1,b_2,b_3,b_4\right\}$. Then we have that $a^- \in \left\{r_1,r_2,r_3,b_5,b_6\right\}$. Let us consider the following cases. 
	\begin{enumerate}
		\item $a^- = r_1$.\\
		Then each agent $b \in \left\{b_1,b_2,b_3,b_4\right\} \setminus \left\{a^n\right\}$ must be in a room that it approves of, i.e., $b \in D_\pi^+$.
		We require at least 2 rooms $S_1,S_2$ with fraction $\frac{1}{3}$ so that each agent in $\left\{b_1,b_2,b_3,b_4\right\} \setminus \left\{a^n\right\}$ is contained in a room with fraction  $\frac{1}{3}$. There is exactly 1 red agent that approves of fraction $\frac{1}{3}$, namely $r_1$. Thus, $S_1$ and $S_2$ both must contain a red agent $r, r' \in R$ that do not approve of fraction $\frac{1}{3}$. Thus, $|D_\pi^-| \geq 2$ as $r,r' \in D_\pi^-$. This contradicts $|D_\pi^-| = 1$.
		
		
		\item $a^- \in \left\{r_2,r_3\right\}$.\\
		W.l.o.g. assume that $a = r_2$. We have that $r_3 \in D_\pi^+$, thus the room $S$ that contains $r_3$ must be of fraction $\frac{2}{3}$. There are exactly 2 agents that approve of fraction $\frac{2}{3}$, namely $r_2$ and $r_3$. Since $r_2 \notin S$, as $r_2 \in D_\pi^-$, the room $S$ must contain a red agent $r \neq r_2$ such that $r \in D_\pi^-$. Thus, $|D_\pi^-| \geq 2$ as $r_2,r \in D_\pi^-$. This contradicts $|D_\pi^-| = 1$.
		
		
		\item $a^- \in \left\{b_5,b_6\right\}$.\\
		Analogous to case 1.\qed
		
	\end{enumerate}
	\end{proof}

\begin{remark}\label{popnot1}
	For outcome $\pi$ of $\overline{G}$, we have that $|D_\pi^-| \geq 1$.
\end{remark}
%\begin{proof}
%	Assume that $|D_\pi^-| = 0$, then we have that $b_5,b_6 \in D_\pi^+$. Therefore, there must exist a room $S$ with fraction $\frac{0}{3}$. There are exactly 2 blue agents that approve of fraction $\frac{0}{3}$, the remaining blue agents disapprove of fraction $\frac{0}{3}$. Thus, $S$ must contain a blue agent that disapproves of the fraction of its assigned room. Therefore, $|D_\pi^-| = 0$ cannot hold. 
%	\qed\end{proof}


\begin{remark}\label{popnot2}
	For outcome $\pi$ of $\overline{G}$, if $|D_\pi^n \cup D_\pi^-| = 2$, then $D_\pi^n \cup D_\pi^- \subseteq \{b_1,b_2,b_3,b_4\}$.
\end{remark}

\begin{lemma}\label{popnotgartopbest}
	Let $\pi$ be an outcome that is not a top-type outcome. There exist a top-type outcome $\pi'$ that is strictly more popular than $\pi$.
\end{lemma}
\begin{proof}
	By \cref{popnotgar2more} we have that $|D_\pi^n \cup D_\pi^-| \geq 2$. By \cref{popnotgartopcard} we have that $|D_\pi^n| \neq 1$ or $|D_\pi^-| \neq 1$. Let us consider the following cases.
	\begin{enumerate}
		\item $|D_\pi^-| \neq 1$.\\
		By \cref{popnot1} and case assumption we have that $|D_\pi^-| \geq 2$. %Consider the following cases.
		\begin{enumerate}[\theenumi.1.]
			\item $|D_\pi^-| = 2$.%\\
			%Consider the following cases.
			\begin{enumerate}[\theenumii1.]
				\item $|D_\pi^n| = 0$.\\
				By \cref{popnot2} we have that $D_\pi^- \subseteq \left\{b_1,b_2,b_3,b_4\right\}$. Let us write $D_\pi^- = \left\{a_1,a_2\right\}$. Since $a_1, a_2 \in \left\{b_1,b_2,b_3,b_4\right\}$, there exists a top-type outcome $\pi'$ such that $D_{\pi'}^- = \left\{a_1\right\}$ and $D_{\pi'}^n = \left\{a_2\right\}$. Thus, $\phi(\pi',\pi) = 1$.
				
				\item $|D_\pi^n| \geq 1$.\\
				Let us write $D_\pi^- = \left\{a_1, a_2\right\}$ and $a_3 \in D_\pi^n$. We have that $a_3 \in \left\{b_1,b_2,b_3,b_4\right\}$. Let $\pi'$ be a top-type outcome such that $\left\{a_3\right\} = D_{\pi'}^n$ and $\left\{a^-\right\} = D_{\pi'}^-$. Note that $N(\pi, \pi') \subseteq \left\{a^-\right\}$.
				\begin{enumerate}[\theenumiii1.]
					\item $N(\pi, \pi') =  \emptyset$.\\
					Then we have that $a^- \in D_\pi^-$. W.l.o.g. assume that $a_1 = a^-$. We have that $a_2 \in D_{\pi'}^+$ and $a_2 \in N(\pi', \pi)$. Thus, $\phi(\pi',\pi) > 0$.
					
					\item $N(\pi, \pi') = \left\{a^-\right\}$.\\
					Then we have that $a^- \in D_\pi^n \cup D_\pi^+$ and $a_1,a_2 \in D_{\pi'}^+$. Thus, $a_1,a_2 \in N(\pi',\pi)$. Therefore, $\phi(\pi',\pi) > 0$.
				\end{enumerate}
			\end{enumerate}
			\item $|D_{\pi}^-| > 2$.\\
			Let us write $a_1, a_2, a_3 \in D_\pi^-$. Let $\pi'$ be an arbitrary top-type outcome with $\left\{a^n\right\} = D_{\pi'}^n$ and $\left\{a^-\right\} = D_{\pi'}^-$. Note that $N(\pi, \pi') \subseteq \left\{a^n, a^-\right\}$. %Consider the following cases.
			\begin{enumerate}[\theenumii1.]
				\item $a^- \in  D_\pi^-$.\\
				W.l.o.g. assume that $a_1 = a^-$. In this case, we have that $N(\pi, \pi') \subseteq \left\{a^n\right\}$. We have that $a_2, a_3 \in N(\pi', \pi)$. Thus, $\phi(\pi', \pi) > 0$. 
				
				\item $a^- \notin  D_\pi^-$.\\
				We have $N(\pi, \pi') \subseteq \left\{a^-, a^n\right\}$ and $a_1, a_2, a_3 \in N(\pi', \pi)$. Thus, $\phi(\pi', \pi) > 0$. 
				
			\end{enumerate}
		\end{enumerate}
		
		\item $|D_{\pi}^n| \neq 1$.
		%Consider the following cases.
		\begin{enumerate}[\theenumi.1.]
			\item $|D_{\pi}^n| = 0$.\\
			By \cref{popnotgar2more}, we have that $|D_{\pi}^-| \geq 2$. This case is the same as case 1.1.1.
			
			\item $|D_{\pi}^n| \geq 2$.\\
			Let us write $a_1, a_2 \in D_\pi^n$. We have that $\left\{a_1, a_2\right\} \subseteq \left\{b_1,b_2,b_3,b_4\right\}$.
			By \cref{popnot1}, we have that $|D_{\pi}^-| \geq 1$. 
			%Let us write $a_3 \in D_\pi^-$. Let us consider the following cases regarding $a_3$.
			\begin{enumerate}[\theenumii1.]
				\item $a_3 \in \left\{b_1,b_2,b_3,b_4\right\}$.\\
				We construct a top-type outcome $\pi'$ such that $D_{\pi'}^- = \left\{a_3\right\}$, $D_{\pi'}^n = \left\{a_2\right\}$, and $a_1 \in D_{\pi'}^+$. We have $N(\pi, \pi') = \emptyset$ and $|N(\pi',\pi)| \geq 1$. Thus, $\phi(\pi', \pi) > 0$.
				
				\item $a_3 \notin \left\{b_1,b_2,b_3,b_4\right\}$.\\
				We construct a top-type outcome $\pi'$ s.t. $D_{\pi'}^- = \left\{a^-\right\}$, $D_{\pi'}^n = \left\{a_1\right\}$, and $a_2, a_3 \in D_{\pi'}^+$. We have $N(\pi,\pi') \subseteq \left\{a^-\right\} \wedge a_2, a_3 \in N(\pi',\pi)$. Thus, $\phi(\pi', \pi) > 0$. \qed
			\end{enumerate}
		\end{enumerate}
	\end{enumerate}
	\end{proof}

\begin{lemma}\label{popnotgartopnonpop}
	A top-type outcome $\pi$ is not popular.
\end{lemma}
\begin{proof}
	Let $\pi$ be a top-type outcome. We can write $\pi = \left\{P_1,P_2,P_3\right\} =$\\
	$\left\{\left\{r_1, \hat{b}_1, \hat{b}_2\right\}, \left\{r_2,r_3,\hat{b}_3\right\}, \left\{b_5,b_6,\hat{b}_4\right\}\right\},$
	where $\hat{b}_1,\hat{b}_2,\hat{b}_3,\hat{b}_4 \in \left\{b_1,b_2,b_3,b_4\right\}$. Let us construct outcome $\pi'$ as follows:
	\begin{align*}
		\pi'=  \left\{P_1 \setminus \left\{\hat{b}_2\right\} \cup \left\{\hat{b}_3\right\}, P_2 \setminus \left\{\hat{b}_3\right\} \cup \left\{\hat{b}_4\right\}, P_3 \setminus \left\{\hat{b}_4\right\} \cup \left\{\hat{b}_2\right\} \right\}
	\end{align*}
	We have that $N(\pi,\pi') = \left\{\hat{b}_2\right\}$ and $N(\pi',\pi) = \left\{\hat{b}_3, \hat{b}_4\right\}$. Thus, $\phi(\pi', \pi) > 0$%Thus, $\pi'$ is strictly more popular than $\pi$.
	\qed\end{proof}

\begin{theorem}
	A popular outcome is not guaranteed to exist in a roommate diversity game $\overline{G}$.
\end{theorem}
\begin{proof}
	From \cref{popnotgartopbest} and \ref{popnotgartopnonpop} we have that no popular outcome exists in $\overline{G}$. Thus, not every roommate diversity game permits a popular outcome.
	\qed\end{proof}

The idea of the co-NP-hardness reduction is to combine the reduction of \cref{mixedpop} with the proof of a popular outcome not being guaranteed to exist. Particularly, the reduced-type outcome is introduced, which is a combination of the reduced outcome and top-type outcome. In this reduction, we have that a popular outcome exists if and only if $(X,C)$ has no solution. The full reduction can be found in the appendix or the full paper.

==> sections/roomsizetwo.tex <==
\section{Room Size Two}
% TODO
% Maybe:
% Make complete graph from agents. Edge weight correspond to rank/distance to neighbor. find min or max weight matching.
